Visualizing the Invisible: A Generative AR System for Intuitive Multi-Modal Sensor Data Presentation

Understanding sensor data can be difficult for non-experts because of the complexity and different semantic meanings of sensor modalities. This leads to a need for intuitive and effective methods to present sensor information. However, creating intuitive sensor data visualizations presents three key challenges: the variability of sensor readings, gaps in domain comprehension, and the dynamic nature of sensor data. To address these issues, we propose Vivar, a novel system that integrates multi-modal sensor data and presents 3D volumetric content for AR visualization. In particular, we introduce a cross-modal embedding approach that maps sensor data into a pre-trained visual embedding space through barycentric interpolation. This approach accurately reflects value changes in multi-modal sensor information, ensuring that sensor variations are properly shown in visualization outcomes. Vivar also incorporates sensor-aware AR scene generation using foundation models and 3D Gaussian Splatting (3DGS) without requiring domain expertise. In addition, Vivar leverages latent reuse and caching strategies to accelerate 2D and AR content generation, demonstrating 11x latency reduction without compromising quality. A user study involving over 503 participants, including domain experts, demonstrates Vivar's effectiveness in accuracy, consistency, and real-world applicability, paving the way for more intuitive sensor data visualization.

==> Mobicom/1-introduction.tex <==
\section{Introduction} 
\label{sec:introduction}

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/t2.jpg}
    \caption{Left: without \pname, sensor data are abstract and hard to be interpreted by non-experts. Right: \pname generates AR scenes with intuitive and immersive sensor data presentation. }
    \label{fig:teaser}
\end{figure}


% \pp{Background - Invisible but Rich Sensing Environment
% \begin{itemize}
%     \item Proliferation of sensors in interconnected world creating invisible data layer
%     \item Sensors capture phenomena beyond human perception (environmental, healthcare, industrial)
%     \item Data is rich in information but abstract and complex
%     \item Barriers exist between valuable sensor data and human understanding
% \end{itemize}
% }
\add{The pervasive deployment of sensors across interconnected networks has generated an extensive, yet largely imperceptible, data layer that captures phenomena beyond human perceptual capabilities~\cite{chataut2023unleashing}. These sensing systems span various domains, including environmental monitoring through multispectral imaging, healthcare through wearable physiological sensors, and industrial applications such as predictive maintenance based on vibrations. However, sensor data itself can be abstract and complex, consisting of numerical readings and technical parameters that lack inherent meaning for individuals without specialized domain knowledge. 
This complexity arises from multiple factors: the nature of the measured phenomena, the technical specifications of the sensors, and the intricate relationships between multiple data streams. Consequently, significant barriers exist that prevent the wealth of information contained within this valuable sensor data from being readily accessible and understood by the general population. The rapid growth in the deployment of connected devices, as illustrated by the projected increase from 16.6 billion in 2023 to 40 billion by 2030 \cite{iot_analytics_2024}, suggests that the challenges associated with interpreting this expanding `invisible data layer' will only become more pronounced. Furthermore, the concentration of these devices in certain geographical regions \cite{demandsage_iot_2024} can lead to disparities in the ability to take advantage of the insights derived from such data.}
\todo{This paragraph does not have any logic. I suggest rolling back to the previous version.}


\add{The challenge of understanding sensory information is particularly difficult for non-experts, who often lack the necessary technical background and domain-specific knowledge to extract meaningful insights. While various approaches exist to aid in data interpretation, visualization has been considered as a particularly useful method for transforming abstract data into more readily understandable forms. Drawing inspiration from the concept of synaesthesia, where stimulation of one sensory modality evokes an experience in another \cite{brang2019double}, we propose that mapping abstract sensor data to intuitive sensory representations, especially visual ones, can significantly enhance comprehension for non-expert users.}

\add{However, traditional data visualization techniques often fall short in making complex sensor data accessible to non-experts. These methods frequently assume a certain level of technical proficiency and domain knowledge, and they can become ineffective when dealing with the scale and complexity characteristic of modern sensor data. The limitations of traditional visualization tools in handling the volume, velocity, and variety of big data are particularly relevant to sensor data, suggesting an inherent constraint in their ability to provide intuitive understanding for general users. Moreover, existing systems often struggle to maintain semantic consistency when integrating and visualizing data from multiple sensors capturing different types of information~\cite{xie2024xdrive}. This lack of consistency across modalities can lead to confusion and hinder accurate interpretation, especially for those without the expertise to reconcile these discrepancies. A fundamental gap remains in creating intuitive connections between the abstract numerical values produced by sensors and their real-world meaning for non-experts. Without these clear links, the data may remain just numbers, devoid of the context and significance necessary for informed decision-making. Psychological perspectives on how individuals process information suggest that non-experts, who may rely more on concrete sensory input, require methods that explicitly bridge this gap between abstract values and intuitive understanding \cite{nearhub_sensing_2025}.} 

\add{Augmented Reality (AR) offers a particularly compelling medium for sensor information visualization to bridge this domain gap. By overlaying digital content onto the physical world, AR provides an immersive and context-aware experience that enhances user interaction with data~\cite{ARapp1, ARapp2}. This capability allows users to intuitively engage with sensor information in their surroundings, turning complex, multimodal data into tangible, interactive experiences. For instance, AR can overlay environmental information such as air quality~\cite{ARairquality}, temperature~\cite{ARtemperature}, or safety conditions~\cite{ARsafetyconditions} directly onto physical spaces, offering a clear and accessible representation of these parameters without requiring specialized expertise. The immersive nature of AR effectively lowers barriers to data interpretation, benefiting both experts and non-experts, as shown in Figure~\ref{fig:teaser}. Presenting sensor information in AR introduces three major challenges: 1) \textit{Variability of Sensor Readings:} Sensor measurements often vary significantly, both individually and in combination. For example, temperature readings may range from -30°C to 40°C, representing vastly different conditions~\cite{temperatureDiverseRange}. Additionally, sensors frequently work together, measuring variables like air quality, temperature, and pollution levels simultaneously~\cite{SensorPollutionMonitoring}, making it challenging to coherently integrate these interrelated data points into a unified scene. 2) \textit{Domain Gap in Comprehension:} The abstract nature of sensor data creates a significant gap in human understanding, requiring tailored visual representations to effectively communicate key features. Bridging this gap often involves long-term study and expert interpretation. 3) \textit{Dynamic Nature of Sensor Data:} The ever-changing nature of sensor readings necessitates just-in-time visualizations that match the rate of data updates, requiring systems capable of rapid interpretation and immediate visual updates.}

\add{Existing sensor data visualization methods face substantial limitations. Traditional dashboards, while effective for domain experts, often prove inaccessible to non-technical users. Recent advances in AI-driven visualization, such as Artificial Intelligence-Generated Content (AIGC) frameworks like Stable Diffusion~\cite{esser2024scaling-sd3}, struggle to seamlessly integrate sensor data as inputs. Similarly, three-dimensional generation methods~\cite{tang2023dreamgaussian, poole2022dreamfusion} show promise but are hindered by high computational demands and limited capability for generating volumetric sensor presentation. These shortcomings highlight the need for a new solution that combines intuitive and immersive user experiences with efficient performance.}

\add{To address these challenges, we propose \pname, a novel system for intuitive and efficient sensor data visualization in AR. Central to \pname is its use of \textbf{barycentric interpolation}~\cite{grunbaum1967convex,angel2005interactive}, a technique inspired by shading principles, to map diverse sensor data into a shared visual embedding space. This interpolation ensures smooth transitions and accurate blending of sensor readings, enabling seamless visualization in both single-sensor and multi-sensor scenarios. The system features an automated, sensor-aware pipeline that generates AR scenes directly from sensor readings, bridging the gap between abstract data and intuitive representation. To manage the rapid dynamics of sensor data, \pname incorporates a latent-reuse mechanism, caching 2D and AR content for timely responsiveness and enhanced efficiency.} We summarize our main contributions as follows:

\begin{enumerate}
    \item \textbf{Cross-modal embedding with barycentric interpolation}: We introduce a novel approach that maps diverse sensor data and combinations into a unified visual embedding space, enabling smooth transitions and improved interpretability.
    \item \textbf{Sensor semantics AR scene generation}: We develop a robust system that automatically generates AR representations from the input of sensor data using foundational models and 3D Gaussian Splatting (3DGS) without requiring domain expertise.
    \item \textbf{Just-in-time efficiency}: We create a fast generation framework with latent-reuse and caching strategies for 2D and AR content that speed the generation up to 10x compared to existing models.
\end{enumerate}

